Aligning Programming Language and Natural Language: Exploring Design Choices in Multi-Modal Transformer-Based Embedding for Bug Localization

Bug localization refers to the identification of source code files which is in a programming language and also responsible for the unexpected behavior of software using the bug report, which is a natural language. As bug localization is labor-intensive, bug localization models are employed to assist software developers. Due to the domain difference between source code files and bug reports, modern bug-localization systems, based on deep learning models, rely heavily on embedding techniques that project bug reports and source code files into a shared vector space. The creation of an embedding involves several design choices, but the impact of these choices on the quality of embedding and the performance of bug localization models remains unexplained in current research. To address this gap, our study evaluated 14 distinct embedding models to gain insights into the effects of various design choices. Subsequently, we developed bug localization models utilizing these embedding models to assess the influence of these choices on the performance of the localization models. Our findings indicate that the pre-training strategies significantly affect the quality of the embedding. Moreover, we discovered that the familiarity of the embedding models with the data has a notable impact on the bug localization model's performance. Notably, when the training and testing data are collected from different projects, the performance of the bug localization models exhibits substantial fluctuations.

==> ALL_MAP.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{landscape}
\newcolumntype{s}{>{\hsize=.26\hsize}X}
\newcolumntype{d}{>{\hsize=.31\hsize}X}
\newcolumntype{l}{>{\hsize=.235\hsize}X}
\newcolumntype{v}{>{\hsize=.11\hsize}X}
\newcolumntype{k}{>{\hsize=.07\hsize}X}
\newcolumntype{q}{>{\centering\hsize=.47\hsize}X}


% \begin{adjustbox}{angle=90,label=table:comparison of embeddings,captionbelow=\textbf{Performance comparison of the embeddings},float={table}[!htbp]}
\begin{table}[]
\caption{MAP of the embedding models.}
\centering
\begin{tabularx}{\linewidth}{|s|d|l|v|k|v|k|k|v|v|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\Name (RQ3)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\Strategy (RQ2)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\Data (RQ1)\end{tabular}}} & \multicolumn{7}{c|}{\textbf{MRR for Test Data}}                                                                                                                                                                                                       \\ \cline{4-10} 
                    &                     &                     & \multicolumn{1}{v|}{\textbf{AspectJ}} & \multicolumn{1}{k|}{\textbf{Birt}} & \multicolumn{1}{v|}{\textbf{Eclipse}} & \multicolumn{1}{k|}{\textbf{JDT}} & \multicolumn{1}{k|}{\textbf{SWT}} & \multicolumn{1}{v|}{\textbf{Tomcat}} & \textbf{Overall} \\ \hline


% \multirow{2}{=}{\textbf{Training Data (for CNN Model)  (RQ1)}}
% \cline{1-10}
% \textbf{Model Name}             & \textbf{Embedding Training Strategy} & \textbf{Training Data (CNN Model)} & \textbf{AspectJ} & \textbf{Birt} & \textbf{Eclipse} & \textbf{JDT} & \textbf{SWT} & \textbf{Tomcat} & \textbf{Overall} \\ \cline{1-10}




\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Long\\ RoBERTa\end{tabular}}                                       & \multirow{2}{*}{Electra}                                                        & BLDS                                                                              & \multicolumn{1}{r|}{0.33}             & \multicolumn{1}{r|}{0.28}          & \multicolumn{1}{r|}{0.28}             & \multicolumn{1}{r|}{0.27}         & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.23}            & 0.26                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.29}             & \multicolumn{1}{r|}{0.21}          & \multicolumn{1}{r|}{0.29}             & \multicolumn{1}{r|}{0.38}         & \multicolumn{1}{r|}{0.31}         & \multicolumn{1}{r|}{0.30}            & 0.28                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{MLM}                                                            & BLDS                                                                              & \multicolumn{1}{r|}{0.17}             & \multicolumn{1}{r|}{0.18}          & \multicolumn{1}{r|}{0.18}             & \multicolumn{1}{r|}{0.25}         & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.16}            & 0.18                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.15}             & \multicolumn{1}{r|}{0.17}          & \multicolumn{1}{r|}{0.22}             & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.28}         & \multicolumn{1}{r|}{0.15}            & 0.17                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{QA}                                                             & BLDS                                                                              & \multicolumn{1}{r|}{0.06}             & \multicolumn{1}{r|}{0.18}          & \multicolumn{1}{r|}{0.12}             & \multicolumn{1}{r|}{0.03}         & \multicolumn{1}{r|}{0.11}         & \multicolumn{1}{r|}{0.15}            & 0.11                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.35}          & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.44}         & \multicolumn{1}{r|}{0.29}         & \multicolumn{1}{r|}{0.36}            & 0.33                                  \\ \hline
\multirow{6}{*}{Reformer}                                           & \multirow{2}{*}{Electra}                                                        & BLDS                                                                              & \multicolumn{1}{r|}{0.23}             & \multicolumn{1}{r|}{0.21}          & \multicolumn{1}{r|}{0.21}             & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.28}         & \multicolumn{1}{r|}{0.20}            & 0.22                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.31}             & \multicolumn{1}{r|}{0.17}          & \multicolumn{1}{r|}{0.25}             & \multicolumn{1}{r|}{0.26}         & \multicolumn{1}{r|}{0.26}         & \multicolumn{1}{r|}{0.20}            & 0.23                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{MLM}                                                            & BLDS                                                                              & \multicolumn{1}{r|}{0.06}             & \multicolumn{1}{r|}{0.07}          & \multicolumn{1}{r|}{0.11}             & \multicolumn{1}{r|}{0.07}         & \multicolumn{1}{r|}{0.09}         & \multicolumn{1}{r|}{0.12}            & 0.07                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.45}             & \multicolumn{1}{r|}{0.25}          & \multicolumn{1}{r|}{0.36}             & \multicolumn{1}{r|}{0.42}         & \multicolumn{1}{r|}{0.34}         & \multicolumn{1}{r|}{0.32}            & 0.35                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{QA}                                                             & BLDS                                                                              & \multicolumn{1}{r|}{0.07}             & \multicolumn{1}{r|}{0.11}          & \multicolumn{1}{r|}{0.12}             & \multicolumn{1}{r|}{0.10}         & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.12}            & 0.09                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.46}             & \multicolumn{1}{r|}{0.35}          & \multicolumn{1}{r|}{0.36}             & \multicolumn{1}{r|}{0.39}         & \multicolumn{1}{r|}{0.35}         & \multicolumn{1}{r|}{0.28}            & 0.36                                  \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Long\\ CodeBERT\end{tabular}}                                      & \multirow{2}{*}{Electra}                                                        & BLDS                                                                              & \multicolumn{1}{r|}{0.36}             & \multicolumn{1}{r|}{0.14}          & \multicolumn{1}{r|}{0.22}             & \multicolumn{1}{r|}{0.25}         & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.12}            & 0.22                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.51}             & \multicolumn{1}{r|}{0.23}          & \multicolumn{1}{r|}{0.35}             & \multicolumn{1}{r|}{0.43}         & \multicolumn{1}{r|}{0.35}         & \multicolumn{1}{r|}{0.33}            & 0.36                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{MLM}                                                            & BLDS                                                                              & \multicolumn{1}{r|}{0.43}             & \multicolumn{1}{r|}{0.30}          & \multicolumn{1}{r|}{0.36}             & \multicolumn{1}{r|}{0.49}         & \multicolumn{1}{r|}{0.25}         & \multicolumn{1}{r|}{0.26}            & 0.36                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.45}             & \multicolumn{1}{r|}{0.37}          & \multicolumn{1}{r|}{0.38}             & \multicolumn{1}{r|}{0.43}         & \multicolumn{1}{r|}{0.27}         & \multicolumn{1}{r|}{0.22}            & 0.37                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{QA}                                                             & BLDS                                                                              & \multicolumn{1}{r|}{0.14}             & \multicolumn{1}{r|}{0.22}          & \multicolumn{1}{r|}{0.23}             & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.13}            & 0.15                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.19}             & \multicolumn{1}{r|}{0.21}          & \multicolumn{1}{r|}{0.26}             & \multicolumn{1}{r|}{0.11}         & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.14}            & 0.16                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{Without training}                                               & BLDS                                                                              & \multicolumn{1}{r|}{0.14}             & \multicolumn{1}{r|}{0.13}          & \multicolumn{1}{r|}{0.15}             & \multicolumn{1}{r|}{0.12}         & \multicolumn{1}{r|}{0.12}         & \multicolumn{1}{r|}{0.20}            & 0.13                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.27}             & \multicolumn{1}{r|}{0.27}          & \multicolumn{1}{r|}{0.27}             & \multicolumn{1}{r|}{0.14}         & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.20}            & 0.21                                  \\ \hline
\multirow{8}{*}{CodeBERT}                                           & \multirow{2}{*}{Electra}                                                        & BLDS                                                                              & \multicolumn{1}{r|}{0.06}             & \multicolumn{1}{r|}{0.18}          & \multicolumn{1}{r|}{0.17}             & \multicolumn{1}{r|}{0.06}         & \multicolumn{1}{r|}{0.18}         & \multicolumn{1}{r|}{0.18}            & 0.10                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.21}             & \multicolumn{1}{r|}{0.15}          & \multicolumn{1}{r|}{0.30}             & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.08}            & 0.19                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{MLM}                                                            & BLDS                                                                              & \multicolumn{1}{r|}{0.27}             & \multicolumn{1}{r|}{0.15}          & \multicolumn{1}{r|}{0.18}             & \multicolumn{1}{r|}{0.26}         & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.17}            & 0.19                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.15}             & \multicolumn{1}{r|}{0.16}          & \multicolumn{1}{r|}{0.22}             & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.09}            & 0.17                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{QA}                                                             & BLDS                                                                              & \multicolumn{1}{r|}{0.09}             & \multicolumn{1}{r|}{0.15}          & \multicolumn{1}{r|}{0.24}             & \multicolumn{1}{r|}{0.08}         & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.12}            & 0.12                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.17}             & \multicolumn{1}{r|}{0.17}          & \multicolumn{1}{r|}{0.21}             & \multicolumn{1}{r|}{0.22}         & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.12}            & 0.17                                  \\ \cline{2-10} 
                                                                    & \multirow{2}{*}{Without training}                                               & BLDS                                                                              & \multicolumn{1}{r|}{0.28}             & \multicolumn{1}{r|}{0.15}          & \multicolumn{1}{r|}{0.17}             & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.09}            & 0.18                                  \\ \cline{3-10} 
                                                                    &                                                                                 & Bench-BLDS                                                                        & \multicolumn{1}{r|}{0.03}             & \multicolumn{1}{r|}{0.17}          & \multicolumn{1}{r|}{0.22}             & \multicolumn{1}{r|}{0.08}         & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.15}            & 0.14                                  \\ \hline
\end{tabularx}
\label{table: map comparison of embeddings}
\end{table}
% \end{adjustbox}
\end{landscape}

==> All_MRR.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{landscape}
\newcolumntype{s}{>{\hsize=.26\hsize}X}
\newcolumntype{d}{>{\hsize=.31\hsize}X}
\newcolumntype{l}{>{\hsize=.235\hsize}X}
\newcolumntype{v}{>{\hsize=.11\hsize}X}
\newcolumntype{k}{>{\hsize=.07\hsize}X}
\newcolumntype{q}{>{\centering\hsize=.47\hsize}X}


% \begin{adjustbox}{angle=90,label=table:comparison of embeddings,captionbelow=\textbf{Performance comparison of the embeddings},float={table}[!htbp]}
\begin{table}[]
\caption{MRR of the embedding models.}
\centering
\begin{tabularx}{\linewidth}{|s|d|l|v|k|v|k|v|v|v|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\Name (RQ3)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\Strategy (RQ2)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Training\\Data (RQ1)\end{tabular}}} & \multicolumn{7}{c|}{\textbf{MRR for Test Data}}                                                                                                                                                                                                       \\ \cline{4-10} 
                    &                     &                     & \multicolumn{1}{v|}{\textbf{AspectJ}} & \multicolumn{1}{k|}{\textbf{Birt}} & \multicolumn{1}{v|}{\textbf{Eclipse}} & \multicolumn{1}{k|}{\textbf{JDT}} & \multicolumn{1}{k|}{\textbf{SWT}} & \multicolumn{1}{v|}{\textbf{Tomcat}} & \textbf{Overall} \\ \hline


% \multirow{2}{=}{\textbf{Training Data (for CNN Model)  (RQ1)}}
% \cline{1-10}
% \textbf{Model Name}             & \textbf{Embedding Training Strategy} & \textbf{Training Data (CNN Model)} & \textbf{AspectJ} & \textbf{Birt} & \textbf{Eclipse} & \textbf{JDT} & \textbf{SWT} & \textbf{Tomcat} & \textbf{Overall} \\ \cline{1-10}




\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Long\\ RoBERTa\end{tabular}}                 & \multirow{2}{*}{Electra}                                   & BLDS                                                         & \multicolumn{1}{r|}{0.41}             & \multicolumn{1}{r|}{0.37}          & \multicolumn{1}{r|}{0.35}             & \multicolumn{1}{r|}{0.37}         & \multicolumn{1}{r|}{0.31}         & \multicolumn{1}{r|}{0.33}            & 0.35                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.37}             & \multicolumn{1}{r|}{0.28}          & \multicolumn{1}{r|}{0.40}             & \multicolumn{1}{r|}{0.49}         & \multicolumn{1}{r|}{0.40}         & \multicolumn{1}{r|}{0.40}            & 0.39                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{MLM}                                       & BLDS                                                         & \multicolumn{1}{r|}{0.28}             & \multicolumn{1}{r|}{0.25}          & \multicolumn{1}{r|}{0.28}             & \multicolumn{1}{r|}{0.33}         & \multicolumn{1}{r|}{0.33}         & \multicolumn{1}{r|}{0.26}            & 0.29                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.24}             & \multicolumn{1}{r|}{0.25}          & \multicolumn{1}{r|}{0.32}             & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.35}         & \multicolumn{1}{r|}{0.25}            & 0.27                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{QA}                                        & BLDS                                                         & \multicolumn{1}{r|}{0.16}             & \multicolumn{1}{r|}{0.27}          & \multicolumn{1}{r|}{0.20}             & \multicolumn{1}{r|}{0.13}         & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.23}            & 0.20                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.42}             & \multicolumn{1}{r|}{0.43}          & \multicolumn{1}{r|}{0.41}             & \multicolumn{1}{r|}{0.54}         & \multicolumn{1}{r|}{0.40}         & \multicolumn{1}{r|}{0.45}            & 0.44                                  \\ \hline
\multirow{6}{*}{Reformer}                     & \multirow{2}{*}{Electra}                                   & BLDS                                                         & \multicolumn{1}{r|}{0.32}             & \multicolumn{1}{r|}{0.29}          & \multicolumn{1}{r|}{0.31}             & \multicolumn{1}{r|}{0.33}         & \multicolumn{1}{r|}{0.37}         & \multicolumn{1}{r|}{0.31}            & 0.32                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.41}             & \multicolumn{1}{r|}{0.26}          & \multicolumn{1}{r|}{0.35}             & \multicolumn{1}{r|}{0.36}         & \multicolumn{1}{r|}{0.32}         & \multicolumn{1}{r|}{0.28}            & 0.33                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{MLM}                                       & BLDS                                                         & \multicolumn{1}{r|}{0.13}             & \multicolumn{1}{r|}{0.18}          & \multicolumn{1}{r|}{0.17}             & \multicolumn{1}{r|}{0.15}         & \multicolumn{1}{r|}{0.18}         & \multicolumn{1}{r|}{0.21}            & 0.17                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.53}             & \multicolumn{1}{r|}{0.34}          & \multicolumn{1}{r|}{0.45}             & \multicolumn{1}{r|}{0.52}         & \multicolumn{1}{r|}{0.42}         & \multicolumn{1}{r|}{0.40}            & 0.44                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{QA}                                        & BLDS                                                         & \multicolumn{1}{r|}{0.16}             & \multicolumn{1}{r|}{0.19}          & \multicolumn{1}{r|}{0.21}             & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.20}         & \multicolumn{1}{r|}{0.22}            & 0.20                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.54}             & \multicolumn{1}{r|}{0.46}          & \multicolumn{1}{r|}{0.46}             & \multicolumn{1}{r|}{0.49}         & \multicolumn{1}{r|}{0.41}         & \multicolumn{1}{r|}{0.36}            & 0.46                                  \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Long\\ CodeBERT\end{tabular}}                & \multirow{2}{*}{Electra}                                   & BLDS                                                         & \multicolumn{1}{r|}{0.45}             & \multicolumn{1}{r|}{0.22}          & \multicolumn{1}{r|}{0.32}             & \multicolumn{1}{r|}{0.33}         & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.20}            & 0.31                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.61}             & \multicolumn{1}{r|}{0.31}          & \multicolumn{1}{r|}{0.42}             & \multicolumn{1}{r|}{0.54}         & \multicolumn{1}{r|}{0.45}         & \multicolumn{1}{r|}{0.41}            & 0.47                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{MLM}                                       & BLDS                                                         & \multicolumn{1}{r|}{0.53}             & \multicolumn{1}{r|}{0.39}          & \multicolumn{1}{r|}{0.46}             & \multicolumn{1}{r|}{0.60}         & \multicolumn{1}{r|}{0.32}         & \multicolumn{1}{r|}{0.36}            & 0.46                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.55}             & \multicolumn{1}{r|}{0.47}          & \multicolumn{1}{r|}{0.46}             & \multicolumn{1}{r|}{0.51}         & \multicolumn{1}{r|}{0.34}         & \multicolumn{1}{r|}{0.29}            & 0.46                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{QA}                                        & BLDS                                                         & \multicolumn{1}{r|}{0.23}             & \multicolumn{1}{r|}{0.31}          & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.20}         & \multicolumn{1}{r|}{0.22}            & 0.26                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.27}             & \multicolumn{1}{r|}{0.28}          & \multicolumn{1}{r|}{0.32}             & \multicolumn{1}{r|}{0.19}         & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.24}            & 0.26                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{Without training}                          & BLDS                                                         & \multicolumn{1}{r|}{0.24}             & \multicolumn{1}{r|}{0.23}          & \multicolumn{1}{r|}{0.21}             & \multicolumn{1}{r|}{0.21}         & \multicolumn{1}{r|}{0.22}         & \multicolumn{1}{r|}{0.28}            & 0.22                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.36}          & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.30}         & \multicolumn{1}{r|}{0.28}            & 0.32                                  \\ \hline
\multirow{8}{*}{CodeBERT}                     & \multirow{2}{*}{Electra}                                   & BLDS                                                         & \multicolumn{1}{r|}{0.13}             & \multicolumn{1}{r|}{0.25}          & \multicolumn{1}{r|}{0.24}             & \multicolumn{1}{r|}{0.14}         & \multicolumn{1}{r|}{0.28}         & \multicolumn{1}{r|}{0.27}            & 0.21                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.28}             & \multicolumn{1}{r|}{0.24}          & \multicolumn{1}{r|}{0.37}             & \multicolumn{1}{r|}{0.26}         & \multicolumn{1}{r|}{0.31}         & \multicolumn{1}{r|}{0.19}            & 0.29                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{MLM}                                       & BLDS                                                         & \multicolumn{1}{r|}{0.36}             & \multicolumn{1}{r|}{0.24}          & \multicolumn{1}{r|}{0.27}             & \multicolumn{1}{r|}{0.34}         & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.26}            & 0.29                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.24}             & \multicolumn{1}{r|}{0.23}          & \multicolumn{1}{r|}{0.30}             & \multicolumn{1}{r|}{0.29}         & \multicolumn{1}{r|}{0.30}         & \multicolumn{1}{r|}{0.20}            & 0.27                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{QA}                                        & BLDS                                                         & \multicolumn{1}{r|}{0.16}             & \multicolumn{1}{r|}{0.24}          & \multicolumn{1}{r|}{0.34}             & \multicolumn{1}{r|}{0.17}         & \multicolumn{1}{r|}{0.22}         & \multicolumn{1}{r|}{0.23}            & 0.23                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.26}             & \multicolumn{1}{r|}{0.24}          & \multicolumn{1}{r|}{0.31}             & \multicolumn{1}{r|}{0.31}         & \multicolumn{1}{r|}{0.29}         & \multicolumn{1}{r|}{0.21}            & 0.28                                  \\ \cline{2-10} 
                                              & \multirow{2}{*}{Without training}                          & BLDS                                                         & \multicolumn{1}{r|}{0.37}             & \multicolumn{1}{r|}{0.25}          & \multicolumn{1}{r|}{0.26}             & \multicolumn{1}{r|}{0.32}         & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.20}            & 0.29                                  \\ \cline{3-10} 
                                              &                                                            & Bench-BLDS                                                   & \multicolumn{1}{r|}{0.13}             & \multicolumn{1}{r|}{0.27}          & \multicolumn{1}{r|}{0.30}             & \multicolumn{1}{r|}{0.17}         & \multicolumn{1}{r|}{0.34}         & \multicolumn{1}{r|}{0.25}            & 0.24                                  \\ \hline

\end{tabularx}
\label{table:comparison of embeddings}
\end{table}
% \end{adjustbox}
\end{landscape}

==> Background.tex <==
\section{Background}
\label{sec-background}
In this section, we will briefly describe some methodologies and transformer-based embedding models which are used in this study.\par
% \subsection{Transfer Learning}
\textbf{Transfer Learning.} Transfer learning is a powerful technique in machine learning that involves leveraging knowledge from one task or domain to improve performance on another related task or domain. The advantages of transfer learning are a fast convergence rate, no need for extensive training datasets, and increased performance. One requirement for this method is that the dataset used in downstream tasks should be similar to the dataset used for pre-training. Using the transfer learning technique, this study used embedding models CodeBERT and LongCodeBERT in the bug localization task. These two embedding models were presented initially as multi-modal embedding trained on source code and code documentation pair and evaluated on code search tasks.
% Usually, neural network weights are initialized randomly. In the transfer learning technique weights, are inherited from another neural network trained on a similar task. The transfer learning technique became popular after using fine-tuning deep neural networks on the Imagenet dataset. Soon, with recent advances, the transfer learning technique was also adopted for natural language processing. It is a process of utilizing existing knowledge for another task in a similar domain. Transfer learning can be used by freezing the initial layers of the model (not updating the weights) and then training the model on a downstream task. The method is appropriate where there is a lack of an extensive training dataset. The advantages of transfer learning are fast convergence rate, no need for extensive training datasets, and increased performance. One requirement for this method is that the dataset used in downstream tasks should be similar to the dataset used for pre-training. This type of semi-supervised training where the neural network is first trained to capture the properties of a language is called language modeling. However, in this study, we have referred to those language models as embedding models. Using the transfer learning technique, this study used embedding models CodeBERT and LongCodeBERT in the bug localization task. These two embedding models were presented initially as multi-modal embedding trained on source code and code documentation pair and evaluated on code search tasks.

% \subsection{Transformer Architectures}
\textbf{Transformer Architectures.} In 2017, Google introduced the Transformer model, a groundbreaking deep learning architecture that leverages attention mechanisms. This approach overcomes the limitations of sequential models like RNNs and LSTMs, which suffer from memory and performance issues when dealing with longer sequences. Bidirectional Encoder Representations from Transformers (BERT) utilizes the transformer architecture, which revolutionized the field of Natural Language Processing (NLP) by achieving state-of-the-art performance across various challenging NLP tasks. It features a multi-layer bidirectional Transformer with 12 transformer layers, 768 hidden units, 12 attention heads, and 110 million trainable parameters. BERT is trained self-supervised, using Masked Language Modeling (MLM) and Next Sentence Prediction (NSP) objectives. While standard BERT models are limited to a maximum sequence length of 512, typical source code files are longer than that. To accommodate this, the researchers proposed Longformer and Reformer, two state-of-the-art BERT architectures capable of supporting sequence lengths up to 4096.

% In  2017,  Google introduced  Transformer,  a type of deep learning model that uses attention mechanism~\citep{Vaswani2017}.  The transformer follows an encoder-decoder architecture. The problem in typical RNN, LSTM based architecture is that the steps in the models are not parallelizable. Thus, they require a significant amount of memory. Moreover, their performance drops drastically if the sequence length is increased. To solve the problem, Vaswani et al.~\citep{Vaswani2017} used an attention mechanism in their model. Later this transformer architecture was used in several other architectures such as  BERT. Google introduced the Bidirectional Encoder Representations from Transformers (BERT) model~\citep{devlin2018bert} that significantly improved state-of-the-art performance for many challenging Natural Language Processing (NLP) tasks. BERT is a multi-layer bidirectional Transformer with an attention mechanism with 12 transformer layers, a hidden size of 768, 12 attention heads, and 110M trainable parameters~\citep{devlin2018bert}. BERT is trained self-supervised using two objectives: Masked Language Modeling(MLM) and Next Sentence Prediction (NSP). In this study, we have used four different embedding models which are based on the architecture of RoBERTa and Reformer. Liu et al. has updated some of the BERT training strategies and tuned hyperparameter in RoBERTa, which leads to performance enhancement. Thus, like previous studies, we also have used RoBERTa. Typical BERT architectures maximum 512 sequence length. However, source code files used to be very long. Longformer and Reformer are some state-of-the-art BERT architecture that can support up to 4096 sequence lengths. Thus, we have chosen  Longformer and Reformer from the long transformer category.

% \subsubsection{RoBERTa}
\begin{itemize}[left=0.1pt]
    \item \textbf{RoBERTa.} Robustly Optimized BERT Pretraining Approach (RoBERTa)~\citep{liu2019} is a variant of the popular BERT model, which uses customized pre-trained methods to improve the BERT transformer model's language understanding. Like the BERT model, the RoBERTa model's input is two sequences of tokens separated by special tokens. In BERT, two tasks are used for training: MLM and NSP. MLM involves predicting replaced tokens, while NSP predicts sentence order. RoBERTa skips NSP and uses a dynamic masking strategy for MLM. Each training data is presented in ten different ways, and hyperparameters are tuned for optimal results.
    \item \textbf{Reformer.} 
    One drawback of BERT-based models is their attention mechanism, which uses dot product attention. This results in memory consumption of $O(L^2)$, where L is the maximum sequence length (e.g., 512 for BERT). However, typical documents or source code files often exceed this limit. To address this issue, Kitaev et al.~\citep{Kitaev2020} introduced the Reformer model with a new attention mechanism called locality-sensitive hashing (LSH) attention. LSH attention reduces the attention calculation cost to $O(L log(L))$ by hashing and storing similar attention. This enables the Reformer model to scale to larger sequence lengths. Kitaev et al. tested their model at a sequence length of 4096 using Wikipedia data.
    
    % One significant drawback of BERT-based models is their attention mechanism. BERT-based transformers use dot product attention. Because of using dot product attention, BERT's memory consumption is $O(L^2)$, where L is the maximum sequence length supported by the model (for BERT, the value of L is 512). High memory consumption in calculating attention hinders BERT-based models from scaling to the higher sequence length. On the other hand, typical natural language documents or source code files are larger than that. To solve this problem, Kitaev et al.~\citep{Kitaev2020} proposed a new attention mechanism in the Reformer model. Instead of dot product-based attention, they proposed locality-sensitive hashing (LSH) attention. In LSH attention, each attention is hashed and stored in the hash container if they have similarities in the hash/local. Thus they reduced the attention calculation cost from $O(L^2)$ to $O(L log(L))$. Thus Reformer model can scale to a larger sequence length. Kitaeve et al. has tested their model at sequence length 4096 using Wikipedia data.
\end{itemize}



% \subsubsection{Reformer}



% \subsection{Training Methodologies}

\textbf{Training Methodologies.} In this study, we used three pre-training methods for language models: Maskled Language Modeling (MLM)~\citep{devlin2018bert}, ELECTRA.~\citep{clark2020electra}, and Question-Answer (QA). MLM~\citep{Lan2019, Zaheer2020, liu2019}, is a common technique that has been widely used in previous studies. ELECTRA is a newer approach that offers faster training and better performance by using a discriminative training strategy. QA was modified in this study to better understand the relationship between bug reports and buggy files. We found that aligning the training technique with the target problem improved language understanding. Therefore, our three pre-training strategies were MLM, QA, and ELECTRA.


% A pre-trained language model is already aware of the basic properties of a language. The pre-trained language model is then fine-tuned using a smaller dataset for downstream tasks like classification, NER (Named Entity Recognition), Question-Answering, etc. In this study for pre-training the embedding models, we followed three methods: MLM, Electra, and QA. The original BERT~\citep{devlin2018bert} includes MLM and NSP pre-training strategies. However, Liu et al.~\citep{liu2019} found that NSP does not improve the language model instead can decrease the performance. Thus we discarded NSP from our pre-training methodologies. On the other hand, Masked Language Model (MLM) is the most common technique to pretrain a language model, which has been used in several previous studies~\citep{Lan2019, Zaheer2020, liu2019}. Thus we have included MLM  in our strategy. Clark et al.~\citep{clark2020electra} proposed a new pre-training task, ELECTRA. ELECTRA is faster than the other techniques and closer to the real-world NLP task. It uses a discriminative approach to train language models, resulting in a better language model. We included ELECTRA in this study as a representative of modern training techniques. The other training technique is Question-Answering (QA). Though QA is a downstream task, we modified the task to understand the relation between a bug report and the buggy file. We found a similarity between the training technique and the bug localization problem. We assumed that the similarity between the training technique and the final problem might improve the language understanding. Thus, we finally got our three pre-training strategies for this study, MLM, QA, and ELECTRA~\citep{clark2020electra}.  

\begin{itemize}[left=0.1pt]
    \item \textbf{MLM:} In Masked Language Modeling (MLM) pre-training, random tokens are masked from the input, and the transformer model learns to predict these masked tokens. However, a problem arises when the special token used for masking doesn't appear in the downstream task, potentially leading to performance degradation. To address this, Devlin et al.~\citep{devlin2018bert} introduced an extra step: randomly selecting tokens with a certain probability and masking a specific portion while replacing others with random tokens. This task aims to minimize the cross-entropy loss in predicting the masked tokens, allowing the transformer model to leverage contextual information. In this study, bug reports and source code were concatenated and used as input for the MLM task.
    
    
    % Random tokens are masked from the input in the Masked Language Modeling (MLM) pre-training strategy, and the transformer model is trained to predict those masked tokens. By the word \emph{masked} we mean some words of the input are replaced by special token $[MASK]$. One problem of this pre-training method is that the special token will not appear in the input in the downstream task. The difference in the input may lead to performance degradation. To mitigate this problem, Devlin et al.~\citep{devlin2018bert} added an extra step. First, tokens are selected randomly with a certain probability. Second,  a specific portion of the selected tokens will be masked others will be replaced by another random token. The goal of this task is to minimize the cross-entropy loss on predicting the masked tokens. It is believed that the transformer model learns to utilize the language's context in this pre-training method. In this study, we concatenated bug reports and source code together and used them as input for the MLM task.
    \item \textbf{QA:} In this technique, the model is trained to locate answers within a given context. We applied this approach to train multi-modal embeddings for bug localization using bug reports and source code files. The bug report serves as the context, and the updated code segment is the answer. By filtering comments and comparing code versions, we obtained questions and contexts for training. We first trained the model using Masked Language Modeling (MLM) and then Question-Answering (QA) to overcome the problem of slow learning.

    
    % In this technique, a pair of questions and context are presented to the model. The answer to the question lies in the context. The transformer model is trained to identify the position of the answer in context. For multi-modal (natural language, programming language) embedding training, we followed this technique. We used bug reports and related source code files to train embeddings. The intuition for using the QA technique in training language models for bug localization is that bug report serves as a context for developers. Developers use the information in a bug report to identify the code segment that needs to be updated. The process is similar to QA, where the bug report is the context, and the updated code segment is the answer. In this training strategy, first, we filtered all comments from the source code. Second, we calculated the difference between before the bug fixing commit and after the bug fixing commit of the buggy source code file. We have speculated that the bug report should contain a direction of bug fixing location in the file, and we have used that as a question. We presented the before-fix version of the source code as a context and the bug report as a question to the transformer. In this method, the transformer is trained to identify the location of the source code edition in the source code file (context). QA task is inherently a bit more complex than MLM task. Previous studies~\citep{shen2018} have reported that if QA has been used as pre-training, the embedding model learns the language comparatively slowly. To overcome that issue, they first trained the embedding model on MLM task and then trained on QA task. We have followed the same approach. However, instead of MLM and QA from now on, we will call this task QA.
    \item \textbf{ELECTRA:} The ELECTRA pre-training method employs a generator and a discriminator. The generator is trained using the Masked Language Modeling (MLM) objective, while the discriminator is trained using the Replaced Token Detection (RTD) objective. It has been observed that the language model trained with the RTD objective outperforms the one trained with the standard MLM objective in downstream tasks. The main difference between MLM and RTD lies in how the loss is calculated: RTD considers all tokens, whereas MLM only focuses on masked tokens. The generator takes the concatenation of bug reports and corresponding code as input, following a specific format. Randomly, 15\% of the tokens are masked, and the generator predicts the replaced tokens. The discriminator, which shares the same architecture as the generator, is trained to classify whether input tokens are replaced or not. In this study, both the generator and discriminator use the same architecture.
    
    
    % The ELECTRA pre-training method uses a generator and a discriminator. The generator is trained using the Masked Language Modeling (MLM) objective, and the discriminator is trained using the Replaced Token Detection(RTD) objective. It has been shown that the language model trained using the RTD objective performs better than the language model trained using the standard MLM objective in downstream tasks \citep{clark2020electra}. One difference between MLM and RTD is that the loss is calculated for all the tokens in the RTD objective, while for the MLM objective, the loss is only calculated for the masked tokens. The MLM objective is to predict the masked tokens. In contrast, the objective of the RTD is to predict whether the individual tokens given as input are replaced or not using the binary classification approach. The input to the generator is the concatenation of the bug report and code corresponding to the bug report. It is of the format $\textlangle s\textrangle$, $W_1$, $W_2$, $W_3$, ..., $W_n$, $\textlangle{}/s\textrangle{}$ and  $\textlangle{} s \textrangle{}$, $C_1$, $C_2$, $C_3$, ..., $C_n$, $\textlangle{}/s\textrangle{}$ where $\textlangle{}s\textrangle{}$ and $\textlangle{}/s\textrangle{}$ are special tokens. 15\% of the tokens are masked randomly by replacing the original tokens with the $\textlangle{}mask\textrangle{}$ token. The generator predicts the tokens that are replaced. The output of the generator is fed to the discriminator. The discriminator is trained to classify whether each of the input tokens is replaced or not. The output of the discriminator is 0 or 1 for each of the input tokens passed. In this study, for generator and discriminator, we have used the same architecture.
\end{itemize}


==> Discussion.tex <==
\section{Discussion}
\label{sec-discussion}

% In this study, we have evaluated the embedding models by their performance in the bug localization task. Our first research question was to verify the necessity of project-specific training for the embedding model. We found that project-specific data can lead to a significant improvement of the generated embeddings. However, training individual bug localization models for individual projects can be costly (both resource and time). Thus this finding emphasizes the importance of the need for research into cross-Project bug localization models.

In this study, we evaluate embedding models by their performance in the bug localization task and found that project-specific training improves embedding quality. However, developing individual models for each project is costly, highlighting the need for research on cross-project bug localization models.
\input{Divergence}
% We have also evaluated the out-of-the-box performance of state-of-the-art multimodal embedding CodeBERT. In most cases, we found that out-of-the-box embedding models' performance was lower than the embedding models trained on bug-localization data. CodeBERT was primarily trained on the code-documentation pair; on the contrary, BLDS and Bench-BLDS contain bug report -source code data. \emph{The observation may point out that for using an embedding in bug localization task, data-specific training is required for the embedding models.} Another point is the performance of the models varies between projects. To investigate the variance, we calculated the difference in token distribution between the BLDS and Bench-BLDS. First, we have tokenized the source codes of the two datasets and calculated the token frequency. Second, we identified the common tokens between the two datasets. Third, we normalized the frequency of the tokens in both datasets. In the final step, we calculated the KL-divergence between BLDS and the Bench-BLDS projects' normalized token frequency. KL divergence~\citep{Kullback1951, wikipedia_2022} measures how different two distributions are. The higher the value, the two distributions are more distant. KL divergence value is equal to zero means that the two distributions are identical. The results are presented in  Table~\ref{table: divergence} along with average performance in the Bench-BLDS projects. From Table~\ref{table: divergence} we can observe that the average performance follows the divergence score. The observation is aligned with the common assumption that the performance will increase if the data used for embedding model training is similar to the test dataset.


We evaluated the  out-of-the-box performance of the CodeBERT embedding model and found that out-of-the-box models perform worse than models trained on bug-localization data. \emph{The observation suggests that specific training with bug report-source code data is necessary for bug localization tasks.} We also noticed performance variance of models across different projects. To identify possible reasons for performance variance, we conducted an analysis of the source codes of different projects. In the analysis, we tokenized and counted the frequency of tokens in both datasets. Then, we found the common tokens and normalized their frequencies. Finally, we calculated the KL-divergence~\citep{Kullback1951, wikipedia_2022} between BLDS and Bench-BLDS projects' token frequencies, which measures the difference between their distributions. Higher values indicate a greater distance between the distributions. The results, shown in Table~\ref{table: divergence}, display the divergence scores alongside the average performance in the Bench-BLDS projects. The table indicates that the average performance follows the divergence score. The observation aligns with the assumption that better performance is expected when the data used for training the embedding model is similar to the test dataset.

% We found that ELECTRA pre-trained models performed better than other pre-training techniques. One of the significant problems of MLM and QA techniques is they do not use the entire document for training. For example, in MLM, only 15\% tokens are randomly selected to be masked. It is less likely that increasing the amount to more than 15\% would be helpful because the embedding model requires context to infer the token that has been masked. ELECTRA utilizes both MLM and replaced token detection (RTD). The generator part learns how to use context in inferring the masked token, while the discriminator learns to differentiate between an original and replaced token. The RTD task utilizes all of the tokens in a document to detect which are replaced. The full utilization of tokens may be one of the reasons why ELECTRA performed better. Moreover, MLM has a fundamental flaw; in training, the embedding model observes a masked token, but there is no masked token in the downstream task (bug localization) or inference. The discrepancy may also contribute to the comparatively poor performance of the MLM pre-trained embedding models.

We found that ELECTRA pre-trained models outperformed other techniques. One problem with MLM and QA techniques is that they don't use the entire document for training. For example, in MLM, only 15\% tokens are randomly selected to be masked. ELECTRA addresses this by combining MLM and replaced token detection (RTD). The generator learns to infer masked tokens using context, while the discriminator distinguishes between original and replaced tokens. RTD utilizes all tokens in a document, potentially contributing to ELECTRA's superior performance. Additionally, MLM has a fundamental flaw as it trains on masked tokens that don't exist in downstream tasks or inference, which may explain the comparatively poorer performance of MLM pre-trained models.

The maximum sequence length supported by typical transformers is small (around 512). The limitation results in the length limitation of embedding models. For example, CodeBERT, PLBART supports sequence lengths 512 and 768, respectively. However, the typical length of source code files is much higher. The limit on the sequence length can be one of the reasons for poor performance. Our findings show that higher sequence length leads to better performance. \emph{The finding may also lead to further study on utilizing small transformers in encoding large source code files.} 

We wondered whether particular bugs are hard to localize. To find the answer to these questions, we have identified easy-to-localize bugs (ranked within the top 7 by all bug localization models) and hard to localize bugs (ranked after $10^{th}$ position by all localization models). We have found that hard to localize bugs has a very long bug description. The median length of the description is 5381, whereas, for easy-to-localize bugs, this length is 631. Moreover, easy to localize bugs contain a comparatively higher percentage of stack trace than easy to localize bugs. \emph{This may indicate that a concise bug report with stack trace may help the bug localization models to perform better.}

% In this study, the bug localization task was defined as a binary classification problem.  We have used a CNN model on top of the embedding models for the classification. However, in some cases, we found that the bare embedding models' performance (using cosine similarity between a bug report and source code) is similar or better than the performance of the bug localization model.

==> Divergence.tex <==
\begin{table}[!tb]
\centering
\caption{Relation between models performance and data similarity.}
\begin{tabular}{|p{2cm}|p{2.5cm}|p{2cm}|}
\hline
\textbf{Project Name} & \textbf{Avg. Performance (MRR)} & \textbf{KL Divergence} \\ \hline
Eclipse Platform UI   & 0.372                           & 1.135                  \\ \hline
AspectJ               & 0.37                            & 1.267                  \\ \hline
JDT                   & 0.367                           & 1.317                  \\ \hline
SWT                   & 0.346                           & 1.369                  \\ \hline
Birt                  & 0.315                           & 1.383                  \\ \hline
Tomcat                & 0.301                           & 1.424                  \\ \hline
\end{tabular}
\label{table: divergence}
\end{table}

==> project_description.tex <==
\begin{table}[!b]
\centering
\caption{Brief description of the projects included in the dataset}
\begin{tabular}{|c|c|}
\hline
\textbf{Project Name} & \textbf{Brief Description}                   \\ \hline
AspectJ               & Programming language                         \\ \hline
Birt                  & Data visualization tool                          \\ \hline
Eclipse UI            & User interfcae framework                     \\ \hline
JDT                   & IDE plugin framework                         \\ \hline
SWT                   & User interface framework                              \\ \hline
Tomcat                & HTTP server                                  \\ \hline
Hadoop                & Distributed processing framework             \\ \hline
Netbeans              & IDE                                          \\ \hline
Storm                 & Distributed computing system                 \\ \hline
Kafka                 & Distributed streaming platform               \\ \hline
Logging-log4j2        & Logging library                              \\ \hline
RxJava                & \begin{tabular}[c]{@{}c@{}}Asynchronous event based\\ programming framework\end{tabular} \\ \hline
Godot                 & Game engine                                  \\ \hline
Guava                 & Java collection library                      \\ \hline
Libgdx                & Game development framework                   \\ \hline
Lucene-solr           & Search library                               \\ \hline
Groovy                & Programming language                         \\ \hline
Elasticsearch         & Distributed search engine                    \\ \hline
Openjpa               & Persistence framework                        \\ \hline
Beam                  & Data streaming library                       \\ \hline
Fresco                & Image manipulation library                   \\ \hline
Jena                  & Semantic web framework                       \\ \hline
Aspnetcore            & Cross-platform web framework                 \\ \hline
Spring-boot           & Web framework                                \\ \hline
Maven                 & Project and dependency management tool       \\ \hline
Ignite                & Distributed database                         \\ \hline
\end{tabular}
\label{table:project_description}
\end{table}
